MANTRA: The Manifold Triangulations Assemblage

The rising interest in leveraging higher-order interactions present in complex systems has led to a surge in more expressive models exploiting higher-order structures in the data, especially in topological deep learning (TDL), which designs neural networks on higher-order domains such as simplicial complexes. However, progress in this field is hindered by the scarcity of datasets for benchmarking these architectures. To address this gap, we introduce MANTRA, the first large-scale, diverse, and intrinsically higher-order dataset for benchmarking higher-order models, comprising over 43,000 and 250,000 triangulations of surfaces and three-dimensional manifolds, respectively. With MANTRA, we assess several graph- and simplicial complex-based models on three topological classification tasks. We demonstrate that while simplicial complex-based neural networks generally outperform their graph-based counterparts in capturing simple topological invariants, they also struggle, suggesting a rethink of TDL. Thus, MANTRA serves as a benchmark for assessing and advancing topological methods, leading the way for more effective higher-order models.

==> figures/betti_example_tetrahedra.tex <==
\begin{figure}[t]
    \center
    \resizebox{0.85\textwidth}{!}{
        \input{figures/img/betti_numbers_example.tex}
    }
    \caption{%
        From left to right,
        %we have 
        four simplicial complexes $\simplicialcomplex_1$,
        $\simplicialcomplex_2$, $\simplicialcomplex_3$, and
        $\simplicialcomplex_4$ with their respective Betti numbers
        $\beta_0$, $\beta_1$, and $\beta_2$. %Recall that the $n$-th
        The $n$-th Betti number indicates the number of $n$-dimensional holes in a
        geometric realization of a simplicial complex.
        Here $\simplicialcomplex_1$ is a solid tetrahedron with
        $\beta_0=1$, $\beta_1=0$, and $\beta_2=0$, since
        $\simplicialcomplex_1$ has only one connected component, no
        unfilled cycles, and no empty cavity enclosed by $2$-faces;
        $\simplicialcomplex_2$ is a hollow tetrahedron with $\beta_0=1$,
        $\beta_1=0$, and $\beta_2=1$ (the difference with
        $\simplicialcomplex_1$ is that the triangles of
        $\simplicialcomplex_2$ enclose a cavity); $\simplicialcomplex_3$
        is the underlying graph, with $\beta_0=1$, $\beta_1=3$, and
        $\beta_2=0$, since there is no cavity and there are three
        linearly independent cycles; $\simplicialcomplex_4$ consists of
        four vertices and has $\beta_0=4$, $\beta_1=0$, and $\beta_2=0$,
        since there are four connected components and no cycles nor
        cavities.}
    \label{fig:tetrahedra_example}
\end{figure}

==> figures/img/betti_numbers_example.tex <==
\begin{tikzpicture}[scale=2]
    % Filled tetrahedron
    \begin{scope}[shift={(-2,0,0)}, rotate around z=20, rotate around y=10]
        \draw[fill=black!30] (0,0,0) -- (1,0,0) -- (0.5,0.866,0) -- cycle;
        \draw[fill=black!40] (0,0,0) -- (1,0,0) -- (0.5,0.289,0.816) -- cycle;
        \draw[fill=black!50] (0,0,0) -- (0.491,0.841,0) -- (0.5,0.289,0.816) -- cycle;
        \draw[fill=black!60] (0,0,0) -- (0.491,0.841,0) -- (0.5,0.289,0.816) -- cycle;

        % Add aligned labels in the upper-right corner
        \node[anchor=west, align=left, rotate=0] at (1.2, 0.25) {$\beta_0=1$ \\ $\beta_1=0$ \\ $\beta_2=0$};
    \end{scope}
    
    % Tetrahedron with lightly filled faces and dashed invisible line
    \begin{scope}[shift={(0,0,0)}, rotate around z=20, rotate around y=10]
        \draw[fill=black!15] (0,0,0) -- (1,0,0) -- (0.5,0.866,0) -- cycle;
        \draw[fill=black!15] (0,0,0) -- (1,0,0) -- (0.5,0.289,0.816) -- cycle;
        \draw[fill=black!15] (0,0,0) -- (0.491,0.841,0) -- (0.5,0.289,0.816) -- cycle;
        \draw[fill=black!15] (0,0,0) -- (0.491,0.841,0) -- (0.5,0.289,0.816) -- cycle;
        \draw[dashed] (0,0,0) -- (1,0,0);
        \draw[dashed] (0,0,0) -- (0.5,0.866,0);
        \draw[dashed] (1,0,0) -- (0.5,0.866,0);
        \node[anchor=west, align=left, rotate=0] at (1.2, 0.25) {$\beta_0=1$ \\ $\beta_1=0$ \\ $\beta_2=1$};
    \end{scope}
    
    % Tetrahedron with only edges
    \begin{scope}[shift={(2,0,0)}, rotate around z=20, rotate around y=10]
        \draw (0,0,0) -- (1,0,0) -- (0.5,0.866,0) -- cycle;
        \draw (0,0,0) -- (0.5,0.289,0.816);
        \draw (1,0,0) -- (0.5,0.289,0.816);
        \draw (0.5,0.866,0) -- (0.5,0.289,0.816);
        \node[anchor=west, align=left, rotate=0] at (1.2, 0.25) {$\beta_0=1$ \\ $\beta_1=3$ \\ $\beta_2=0$};
    \end{scope}
    
    % Tetrahedron with only vertices
    \begin{scope}[shift={(4,0,0)}, rotate around z=20, rotate around y=10]
        \fill (0,0,0) circle (0.05);
        \fill (1,0,0) circle (0.05);
        \fill (0.5,0.866,0) circle (0.05);
        \fill (0.5,0.289,0.816) circle (0.05);
        \node[anchor=west, align=left, rotate=0] at (1.2, 0.25) {$\beta_0=4$ \\ $\beta_1=0$ \\ $\beta_2=0$};
    \end{scope}
\end{tikzpicture}

==> figures/vizualize_random_node_features.tex <==
\begin{figure}[t]
    \center
    \includegraphics[width=.19\textwidth]{./figures/manifolds/render_manifold_2_4_1.png}%
    \includegraphics[width=.19\textwidth]{./figures/manifolds/render_manifold_2_7_1.png}%
    \includegraphics[width=.19\textwidth]{./figures/manifolds/render_manifold_2_6_1.png}%
    \includegraphics[width=.19\textwidth]{./figures/manifolds/render_manifold_2_7_2.png}%
    \includegraphics[width=.19\textwidth]{./figures/manifolds/render_manifold_2_7_4.png}%
    \caption{%
        Geometric realizations of some manifold triangulations included in
        MANTRA.
        %
        %It is usual to think of a manifold triangulation as a nicely
        %embedded simplicial complex on the associated manifold, where the
        %position and coordinates of the simplices are meaningful. 
        %
        The precise coordinates of vertices in Euclidean space are not
        geometrically significant; what matters is the topology of the
        resulting polyhedra.
        %
        % However, realizations of triangulations may not be geometrically
        % informative, as we simply require a homeomorphism between the
        % realization and the original manifold. Due to the small quantity
        % of vertices used to triangulate the manifolds of MANTRA, its
        % triangulations do not contain significant geometric information
        % about their associated manifolds, making MANTRA a purely
        % combinatorial dataset.
        %
        Hence, MANTRA is a \emph{purely combinatorial dataset}.%
    }%
    \label{fig:projected_triangulations}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Backup 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
%
% \begin{figure}[t]
%     \center
%     \includegraphics[width=\textwidth]{./figures/img/random_node_features.png}
%     %\caption{Projected 
%     \caption{%
%         Geometric realizations of some manifold triangulations included in
%         MANTRA.
%         %
%         %It is usual to think of a manifold triangulation as a nicely
%         %embedded simplicial complex on the associated manifold, where the
%         %position and coordinates of the simplices are meaningful. 
%         %
%         The precise coordinates of vertices in Euclidean space are not
%         geometrically significant; what matters is the topology of the
%         resulting polyhedra.
%         %
%         % However, realizations of triangulations may not be geometrically
%         % informative, as we simply require a homeomorphism between the
%         % realization and the original manifold. Due to the small quantity
%         % of vertices used to triangulate the manifolds of MANTRA, its
%         % triangulations do not contain significant geometric information
%         % about their associated manifolds, making MANTRA a purely
%         % combinatorial dataset.
%         %
%         Hence, MANTRA is a \emph{purely combinatorial dataset}.%
%     }%
%     \label{fig:projected_triangulations}
% \end{figure}
%
%


==> tables/dataset_field_description.tex <==
%
%\begin{table}[h!]
{%
	\centering%
	\newcolumntype{D}[1]{>{\small \tt \let\newline\\\arraybackslash\hspace{0pt}}m{#1}}%
	\newcolumntype{C}[1]{>{\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}%
	%\label{tab:DatasetDescription}
	%\resizebox{\linewidth}{!}{
  \begin{tabularx}{\linewidth}{@{}llX}
		\toprule
		{\sc\small Field}                  & {\sc\small Type} & {\sc Description}                                                                                                                                                                                                      \\\midrule
		{\tt\small id}                     & {\tt\small str}  & This attribute refers to the original ID of the triangulation as used by~\cite{manifold_page} when compiling the triangulations. This facilitates comparisons to the original dataset if necessary.                    \\                                                                                                                                                        
		{\tt\small triangulation}          & {\tt\small list} & A doubly-nested list of the facets of the  triangulation.                                                                                                                                                              \\
		{\tt\small n\_vertices}            & {\tt\small int}  & The number of vertices in the triangulation.                                                                                                                                                                           \\
		{\tt\small name}           &  {\tt\small str} 
		                           &  Homeomorphism type of the triangulation. 
		                              Possible values are \texttt{\uq{}\uq}, \texttt{\uq{}Klein bottle\uq}, \texttt{\uq{}RP\^{}{}2\uq}, \texttt{\uq{}S\^{}2\uq}, \texttt{\uq{}T\^{}2\uq{}} for surfaces, where \texttt{\uq{}\uq} indicates that the explicit homeomorphism type is  not available. 
		                              For $3$-dimensional manifolds, possible values are  
		                              \texttt{\uq{}S\^{}2 twist S\^{}1\uq}, \texttt{\uq{}S\^{}2 x   S\^{}1\uq}, 
		                              \texttt{\uq{}S\^{}3\uq}. \\ 
		{\tt\small betti\_numbers}         & {\tt\small list} & A list  of Betti numbers of the triangulation, computed using   $\ring=\integers$, i.e., integer coefficients.                                                                                                     \\
		{\tt\small torsion\_coefficients} & {\tt\small list} & A list of the torsion subgroups of the triangulation.  Possible values are \texttt{\uq{}\uq}, \texttt{\uq{}Z\_2\uq}, where an  empty string \texttt{\uq{}\uq} indicates that no torsion is present in  that dimension. \\
    {\tt\small genus} & {\tt\small int} & For surfaces, contains the genus  of the triangulation. \\
    {\tt\small orientable} & {\tt\small bool} &  For surfaces, specifies if the triangulation is orientable or not. \\ 
		\bottomrule
	\end{tabularx}%
	%}%
}


==> tables/graph_versus_topology_full.tex <==
\begin{table}[t]
	\sisetup{
		detect-all              = true,
		table-format            = 2.2(2),
		separate-uncertainty    = true,
		retain-zero-uncertainty	= true,
		round-mode              = places,
		round-precision         = 2,
		minimum-decimal-digits  = 2,
	}%
	\caption{
		Predictive performance of graph- and simplicial complex-based models on surface and $3$-manifold tasks.
		%
		Results for the full set of surfaces ($2\dash\mathcal{M}^0$), for the set
		of surfaces with known homeomorphism type ($2\dash\mathcal{M}^0_H$), and for the full
		set of three-manifolds ($3\dash\mathcal{M}^0$) are reported. Additionally, performance metrics
		for the barycentric subdivision of the test set on the models trained on
		$2\dash\mathcal{M}^0_H$, i.e.\@, $2\dash\mathcal{M}^1_H$, are included; see
		Section~\ref{scn:barycentric_subdivision_exps} for details.
		For each family of models, $\mathcal{G}$ (graph-based) and $\mathcal{T}$ (simplicial complex-based), we report the mean
		and standard deviation of the maximum performance achieved across five runs by
		each combination of feature vector initialization and model contained in the family.
		The tasks reported are prediction of $\beta_0$, $\beta_1$, $\beta_2$, $\beta_3$, prediction of the
		homeomorphism type, and prediction of orientability.
		%
		For all tasks except for prediction of~$\beta_0$, we report the AUROC metric.
		%
		For $\beta_0$, we report accuracy.
		%
		% Metrics are multiplied by $100$ and rounded to the second decimal for a better visualization.
		%
		%Homeo.\ type and acc. stands for homeomorphism type and accuracy, respectively. 
		%
		Best average result among both families for each task is in bold.
		%
		%Benchmarks on three dataset types are reported. $2$-$\mathcal{M}^0$ refers to using all surfaces,
		%$2$-$\mathcal{M}^0_H$ to all surfaces with a homeomorphism type label, and $2$-$\mathcal{M}^1_H$ to 
		%$2$-$\mathcal{M}_H$ with one barycentric subdivision. For the Betti 
		%numbers, the $i$'th value column corresponds to the $i$'th Betti number 
		%$\beta_i$. $\mathcal{G}$ denotes the family of graph-based 
		%models and $\mathcal{T}$ the simplicial complex-based models, respectively.
		%
		Note that the reported averages and standard deviations are not calculated from individual model performances across different random seeds.
		%
		Instead, for each model, we selected its best performance achieved across all seeds for each experiment.
		%
		Then, we aggregated these best performances within each category—graph-based and simplicial complex-based models—to compute the averages and standard deviations reported in the table.
	}%
	\vspace{.5em}
	\resizebox{\textwidth}{!}{
		\label{tab:graphbased_versus_topological}
		\begin{tabular}{lc SS SS SS}
			\toprule
			                                       &                          & {\it Accuracy}           & \multicolumn{5}{c}{\it AUROC}                                                                                                              \\
			\midrule
			{\small\sc Dataset}                    & {\small\sc Model Family} & {\small $\beta_0$}       & {\small $\beta_1$}            & {\small $\beta_2$}       & {\small $\beta_3$}       & {\small\sc Homeo. Type}  & {\small\sc Orientability} \\
			\midrule
			\multirow[c]{2}{*}{$2\dash\M^{0}$}     & {\G}                     & \bfseries 1.0 \pm 0.0    & 0.5 \pm 0.0                   & 0.5 \pm 0.0              &                          & 0.47 \pm 0.01            & 0.5 \pm 0.0               \\
			                                       & {\T}                     & 0.73 \pm 0.39            & \bfseries  0.68 \pm 0.16      & \bfseries  0.59 \pm 0.1  &                          & \bfseries  0.69 \pm 0.18 & \bfseries  0.56 \pm 0.07  \\
                                             \midrule
			\multirow[c]{2}{*}{$2\dash\M_{H}^{0}$} & {\G}                     & \bfseries  1.0 \pm 0.0   & 0.21 \pm 0.0                  & 0.5 \pm 0.0              &                          & 0.49 \pm 0.01            & 0.5 \pm 0.0               \\
			                                       & {\T}                     & 0.57 \pm 0.44            & \bfseries  0.25 \pm 0.03      & \bfseries  0.52 \pm 0.02 &                          & \bfseries  0.66 \pm 0.13 & \bfseries  0.52 \pm 0.02  \\
                                             \midrule
			\multirow[c]{2}{*}{$2\dash\M_{H}^{1}$} & {\G}                     & \bfseries  0.47 \pm 0.51 & 0.22 \pm 0.0                  & 0.5 \pm 0.0              &                          & 0.49 \pm 0.04            & 0.5 \pm 0.0               \\
			                                       & {\T}                     & 0.21 \pm 0.38            & \bfseries  0.25 \pm 0.02      & \bfseries  0.51 \pm 0.01 &                          & \bfseries  0.6 \pm 0.1   & \bfseries  0.51 \pm 0.01  \\
                                             \midrule
			\multirow[c]{2}{*}{$3\dash\M^{0}$}     & {\G}                     & \bfseries  1.0 \pm 0.0   & 0.23 \pm 0.0                  & 0.12 \pm 0.0             & 0.14 \pm 0.0             &                          & 0.14 \pm 0.0              \\
			                                       & {\T}                     & 0.78 \pm 0.41            & \bfseries  0.25 \pm 0.04      & \bfseries  0.13 \pm 0.03 & \bfseries  0.16 \pm 0.03 &                          & \bfseries  0.15 \pm 0.02  \\
			\bottomrule
		\end{tabular}
	}
\end{table}

%
%
% \multirow[c]{2}{*}{F2D}  & \multirow[c]{2}{*}{0.000000} & Graph        & 1.0 \pm 0.0   & 0.5 \pm 0.0   & 0.5 \pm 0.0   &               & 0.47 \pm 0.01   & 0.5 \pm 0.0     \\
%                          &                              & Topological  & 0.66 \pm 0.41 & 0.73 \pm 0.14 & 0.61 \pm 0.1  &               & 0.75 \pm 0.15   & 0.57 \pm 0.07   \\
% \multirow[c]{4}{*}{NN2D} & \multirow[c]{2}{*}{0.000000} & Graph        & 1.0 \pm 0.0   & 0.21 \pm 0.0  & 0.5 \pm 0.0   &               & 0.51 \pm 0.01   & 0.5 \pm 0.0     \\
%                          &                              & Topological  & 0.46 \pm 0.42 & 0.26 \pm 0.03 & 0.53 \pm 0.02 &               & 0.71 \pm 0.11   & 0.53 \pm 0.02   \\
%                          & \multirow[c]{2}{*}{1.000000} & Graph        & 0.47 \pm 0.51 & 0.22 \pm 0.0  & 0.5 \pm 0.0   &               & 0.49 \pm 0.04   & 0.5 \pm 0.0     \\
%                          &                              & Topological  & 0.21 \pm 0.38 & 0.25 \pm 0.02 & 0.51 \pm 0.01 &               & 0.6 \pm 0.1     & 0.51 \pm 0.01   \\
% \multirow[c]{2}{*}{F3D}  & \multirow[c]{2}{*}{0.000000} & Graph        & 1.0 \pm 0.0   & 0.24 \pm 0.0  & 0.12 \pm 0.0  & 0.15 \pm 0.0  &                 & 0.15 \pm 0.0    \\
%                          &                              & Topological  & 0.72 \pm 0.44 & 0.25 \pm 0.04 & 0.14 \pm 0.03 & 0.17 \pm 0.03 &                 & 0.15 \pm 0.02   \\
%


==> tables/graph_versus_topology_full_stage.tex <==
\begin{tabular}{llllllll}
	{}                        & {task}       & {Betti 0}     & {Betti 1}     & {Betti 2}     & {Betti 3}     & {Homeomorphism} & {Orientability} \\
	{}                        & {metric}     & {Accuracy}    & {AUROC}       & {AUROC}       & {AUROC}       & {AUROC}         & {AUROC}         \\
	{dataset}                 & {modelclass} & {}            & {}            & {}            & {}            & {}              & {}              \\
	\multirow[c]{2}{*}{F2D0}  & Graph        & 1.0 \pm 0.0   & 0.5 \pm 0.0   & 0.5 \pm 0.0   &               & 0.47 \pm 0.01   & 0.5 \pm 0.0     \\
	                          & Topological  & 0.73 \pm 0.39 & 0.68 \pm 0.16 & 0.59 \pm 0.1  &               & 0.69 \pm 0.18   & 0.56 \pm 0.07   \\
	\multirow[c]{2}{*}{NN2D0} & Graph        & 1.0 \pm 0.0   & 0.21 \pm 0.0  & 0.5 \pm 0.0   &               & 0.49 \pm 0.01   & 0.5 \pm 0.0     \\
	                          & Topological  & 0.57 \pm 0.44 & 0.25 \pm 0.03 & 0.52 \pm 0.02 &               & 0.66 \pm 0.13   & 0.52 \pm 0.02   \\
	\multirow[c]{2}{*}{NN2D1} & Graph        & 0.47 \pm 0.51 & 0.22 \pm 0.0  & 0.5 \pm 0.0   &               & 0.49 \pm 0.04   & 0.5 \pm 0.0     \\
	                          & Topological  & 0.21 \pm 0.38 & 0.25 \pm 0.02 & 0.51 \pm 0.01 &               & 0.6 \pm 0.1     & 0.51 \pm 0.01   \\
	\multirow[c]{2}{*}{F3D0}  & Graph        & 1.0 \pm 0.0   & 0.23 \pm 0.0  & 0.12 \pm 0.0  & 0.14 \pm 0.0  &                 & 0.14 \pm 0.0    \\
	                          & Topological  & 0.78 \pm 0.41 & 0.25 \pm 0.04 & 0.13 \pm 0.03 & 0.16 \pm 0.03 &                 & 0.15 \pm 0.02   \\
\end{tabular}


==> tables/triangulation_classification.tex <==
\begin{wraptable}{l}{0.25\textwidth}
  \vspace{-1\baselineskip}
	\centering
	\sisetup{
		detect-all              = true,
		table-format            = 5.0,
		separate-uncertainty    = true,
		retain-zero-uncertainty = true,
	}% 
	\caption{%
		Number of triangulations by manifold dimension 
		($2\dash\mathcal{M}$: $2$-manifolds; $3\dash\mathcal{M}$: $3$-manifolds) 
		and number
		of vertices $\vert V \vert$ in a triangulation.%
	}%
	\label{tbl:triangulation_classification_by_vertices}%
  \resizebox{\linewidth}{!}{
    \begin{tabular}{S[table-format=2]S[table-format=5.0]S[table-format=6.0]}
			\toprule
      {$\vert V \vert $} & {$2\dash\mathcal{M}$} & {$3\dash\mathcal{M}$} \\
			\midrule
			4                & 1               & 0               \\
			5                & 1               & 1               \\
			6                & 3               & 2               \\
			7                & 9               & 5               \\
			8                & 43              & 39              \\
			9                & 655             & 1297           \\
			10               & 42426           & 249015          \\
			\midrule
      {Total}            & 43138           & 250359          \\
			\bottomrule
		\end{tabular}
  }
\end{wraptable}

